Issues with Input-Space Representation in Nonlinear Data-Based Dissipativity Estimation

In data-based control, dissipativity can be a powerful tool for attaining stability guarantees for nonlinear systems if that dissipativity can be inferred from data. This work provides a tutorial on several existing methods for data-based dissipativity estimation of nonlinear systems. The interplay between the underlying assumptions of these methods and their sample complexity is investigated. It is shown that methods based on delta-covering result in an intractable trade-off between sample complexity and robustness. A new method is proposed to quantify the robustness of machine learning-based dissipativity estimation. It is shown that this method achieves a more tractable trade-off between robustness and sample complexity. Several numerical case studies demonstrate the results.

==> Sections/Complexity.tex <==
\begin{itemize}
    \item Standard method for robust dissipativity estimation requires a covering radius for the input space
    \item For a constant radius, the sample complexity is super-exponential in the basis dimension
    \item This sample complexity results in super-exponential time and space complexity with existing methods
    \item Probabilistic sampling provides little asymptotic benefit
    \item Alternative approach yields similar results with super-exponential time complexity and constant space complexity
    \item Quantum computing can trade between super-exponential time and space complexity, but not both.
    \item Conclusion is that sampling on a large number of basis functions is impractical
\end{itemize}

==> Sections/Introduction_old.tex <==





This section introduces the existing state of the art and provides context for the work that follows. It will cite a lot of things \cite{Montenbruck2016}. It will also state the main contributions of this work.

Most importantly, we will point out that while dissipativity-based tools for analysis and design have been around for over 60 years, their application has been limited to toy problems or particular special cases. A few examples. Why is this? Though dissipativity has the flexibility to describe complex nonlinear systems in useful ways, finding and verifying such a description is generally quite difficult. Much progress has been made for dissipativity analysis of linear systems and linear systems with specific nonlinearities, like delay or parameteric uncertainty. Cite. For more general nonlinearities, dissipativity can be found analytically, but there is no constructive method, so doing so is about as challenging as finding a Lyapunov function. This is quite hard for any nonlinear system with more than one input-output pair and a few states. 

Any properly interesting system will have nonlinearities not falling in a neat category, and it will be much higher-dimensional than can be approached by hand. Estimating dissipativity from data is a compelling idea in such cases, and there has been much work developing these techniques in the literature. These methods have been promising on toy problems in small dimensions; however, again they appear to suffer similar limitations due to the sheer volume of data and number of computations required to achieve a reasonable estimate.

Dissipativity is a property that must hold for all possible inputs to a system. This is usually taken to mean all finite energy signals, $\mathcal{L}_2$ (or $\ell_2$ for discrete sequences). Taking advantage of linearity, an LTI system's behavior can be completely characterized by its response to pure sinusoids of every frequency. This has long been a tractable data-based approach to system characterization via experimental Bode and Nyquist plots. More recently, Willems' Fundamental Lemma [cite Willems] shows that a single persistently exiting input signal is sufficient to fully characterize an LTI system's behavior [cite Romer]. For nonlinear systems, neither of these simplifications hold, so the input space much be searched in its entirety for a worst-case behavior. Consequently, it is necessary to restrict the input space to a finite set. Ubiquitously in robust nonlinear dissipativity estimation, the approach is as follows:
\begin{enumerate}
\item restrict $\mathcal{L}_2$ in time and magnitude
\item represent the restricted $\mathcal{L}_2$ with a set of basis functions
\item limit the number of basis functions allowed in the input space
\end{enumerate}
Typically, the basis functions have been Fourier or Legendre functions, and the justification has been that inputs above a certain frequency are negligable. In this work, we show that this method is computationally intractable with more than a few basis functions, and using only a few basis functions to represent $\mathcal{L}_2$ results misleading conclusions, even for very simple LTI systems.
